Counting Stacked Objects

Visual object counting is a fundamental computer vision task underpinning numerous real-world applications, from cell counting in biomedicine to traffic and wildlife monitoring. However, existing methods struggle to handle the challenge of stacked 3D objects in which most objects are hidden by those above them. To address this important yet underexplored problem, we propose a novel 3D counting approach that decomposes the task into two complementary subproblems - estimating the 3D geometry of the object stack and the occupancy ratio from multi-view images. By combining geometric reconstruction and deep learning-based depth analysis, our method can accurately count identical objects within containers, even when they are irregularly stacked. We validate our 3D Counting pipeline on diverse real-world and large-scale synthetic datasets, which we will release publicly to facilitate further research.

==> figs/challenging.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{figure}[ht]
    \centering
        \includegraphics[width=0.49\linewidth]{images/challenging/rice.jpg}
        \includegraphics[width=0.49\linewidth]{images/challenging/rice_view.jpg}
        \caption{\textbf{Partial view.} Since our method is designed to be robust to restricted views of the objects to count, it is able to infer an accurate occupancy ratio from small openings in packaging, such as in the \textit{rice} scene (\textit{Est}. 21649, \textit{G.T.} 20063 (approx.), $\gamma_{est}=43.1\%$).}
         
          \label{fig:partial}
\end{figure}

%-------
% OLD
%-------

\iffalse

\begin{figure*}[ht]
    \centering
    
    % First pair: Rice images
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=0.49\textwidth]{images/challenging/rice.jpg}
        \includegraphics[width=0.49\textwidth]{images/challenging/rice_view.jpg}
        \caption{\textbf{Partial view.} Since our method is designed to be robust to restricted views of the objects to count, it is able to infer an accurate occupancy ratio from small openings in packaging, such as in the \textit{rice} scene (\textit{Est}. 21649, \textit{G.T.} 20000, $\gamma_{est}=43.1\%$). \CD{But the user needs to select that area of interest in the image (for now). How to subtly mention this limitation?}}
    \end{subfigure}
    \hfill
    % Second pair: Pasta and pins images
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=0.49\textwidth]{images/challenging/pasta.jpg}
        \includegraphics[width=0.49\textwidth]{images/challenging/pins.jpg}
        \caption{\textbf{Failure cases.} For some highly complex shapes, our method fails to predict an accurate $\gamma_{est}$. They are represented in our real dataset, such as the scenes \textit{pasta} (\textit{Est}. 2025, \textit{G.T.} 588, $\gamma_{est}=23.9\%$) and \textit{pins} (\textit{Est}. 100, \textit{G.T.} 205, $\gamma_{est}=15.9\%$).}
    \end{subfigure}
    
    \caption{\textbf{Challenging scenes from our dataset.} Examples of challenging object counting scenarios.}
    \label{fig:challenging}
\end{figure*}

\fi



==> figs/supp_real_samples.tex <==
\newcommand{\names}{beans,chickpeas,chocolates,crosses,crosses2,gums2,popcorn,puzzle,screws,screws2,semicrosses,semicrosses2}

\newcommand{\counts}{161,2668,201,40,317,500,2229,574,295,627,156,196}
\newcommand{\gts}{207,3276,131,205,205,397,2921,1000,514,494,257,257}






\begin{figure}[ht]
    \centering
    % Top row with RGB images and input names
    %\foreach \input in \inputnames {%
    \foreach \name [count=\j from 0] in \names {
        \pgfmathparse{array({\counts},{\j})} % Extract the j-th count
        \edef\count{\pgfmathresult}
        \pgfmathparse{array({\gts},{\j})} % Extract the j-th count
        \edef\gt{\pgfmathresult}
        \begin{minipage}[c]{0.32\linewidth} % Adjust width for spacing
            \centering
            %\textbf{\input} \vspace{0.2em} \\ % Input name at the top of each column
            %\includegraphics[width=\textwidth]{images/samples/00000392_RGB.png}
            \includegraphics[width=\textwidth]{images/supp_real/\name.jpg}
            \vspace{-2em}\caption*{\centering\textit{\name}:\\\textit{Est.} \count,  \\\textit{G.T.} \gt}\vspace{0.5em}
        \end{minipage}\hspace{-0.5em}%
    }

    \caption{\textbf{Additional dataset samples.} We report the results on all real scenes that are not already present in our main submission.}
    \label{fig:additional_real_samples}
\end{figure}



\iffalse

DOUBLE COLUMN 

\begin{figure*}[ht]
    \centering
    % Top row with RGB images and input names
    %\foreach \input in \inputnames {%
    \foreach \name [count=\j from 0] in \names {
        \pgfmathparse{array({\counts},{\j})} % Extract the j-th count
        \edef\count{\pgfmathresult}
        \pgfmathparse{array({\gts},{\j})} % Extract the j-th count
        \edef\gt{\pgfmathresult}
        \begin{minipage}[c]{0.23\textwidth} % Adjust width for spacing
            \centering
            %\textbf{\input} \vspace{0.2em} \\ % Input name at the top of each column
            %\includegraphics[width=\textwidth]{images/samples/00000392_RGB.png}
            \includegraphics[width=\textwidth]{images/supp_real/\name.jpg}
            \vspace{-2em}\caption*{\centering\textit{\name}:\\\textit{Est.} \count,  \textit{G.T.} \gt}\vspace{1em}
        \end{minipage}%
    }

    \caption{\textbf{Additional dataset samples.} We report the results on all real scenes that are not already present in our main submission.}
    \label{fig:additional_real_samples}
\end{figure*}

\fi
